Reconstruction and Performance Evaluation of FASER's Emulsion Detector at the LHC

This paper presents the reconstruction and performance evaluation of the FASER$\nu$ emulsion detector, which aims to measure interactions from neutrinos produced in the forward direction of proton-proton collisions at the CERN Large Hadron Collider. The detector, composed of tungsten plates interleaved with emulsion films, records charged particles with sub-micron precision. A key challenge arises from the extremely high track density environment, reaching $\mathcal{O}(10^5)$ tracks per cm$^2$. To address this, dedicated alignment techniques and track reconstruction algorithms have been developed, building on techniques from previous experiments and introducing further optimizations. The performance of the detector is studied by evaluating the single-film efficiency, position and angular resolution, and the impact parameter distribution of reconstructed vertices. The results demonstrate that an alignment precision of 0.3 micrometers and robust track and vertex reconstruction are achieved, enabling accurate neutrino measurements in the TeV energy range.

==> authorlist250404_plus.tex <==
\author{Roshan Mammen Abraham\,\orcidlink{0000-0003-4678-3808}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Xiaocong Ai\,\orcidlink{0000-0003-3856-2415}}
\affiliation{School of Physics, Zhengzhou University, Zhengzhou 450001, China}

\author{Saul Alonso Monsalve\,\orcidlink{0000-0002-9678-7121}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

\author{John Anders\,\orcidlink{0000-0002-1846-0262}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Claire Antel\,\orcidlink{0000-0001-9683-0890}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Akitaka Ariga\,\orcidlink{0000-0002-6832-2466}}
\affiliation{Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics, University of Bern, Sidlerstrasse 5, CH-3012 Bern, Switzerland}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Tomoko Ariga\,\orcidlink{0000-0001-9880-3562}}
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Jeremy Atkinson\,\orcidlink{0009-0003-3287-2196}}
\affiliation{Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics, University of Bern, Sidlerstrasse 5, CH-3012 Bern, Switzerland}

\author{Florian~U.~Bernlochner\,\orcidlink{0000-0001-8153-2719}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Tobias Boeckh\,\orcidlink{0009-0000-7721-2114}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Jamie Boyd\,\orcidlink{0000-0001-7360-0726}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Lydia Brenner\,\orcidlink{0000-0001-5350-7081}}
\affiliation{Nikhef National Institute for Subatomic Physics, Science Park 105, 1098 XG Amsterdam, Netherlands}

\author{Angela Burger\,\orcidlink{0000-0003-0685-4122}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Franck Cadoux} % No ORCID
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Roberto Cardella\,\orcidlink{0000-0002-3117-7277}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{David~W.~Casper\,\orcidlink{0000-0002-7618-1683}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Charlotte Cavanagh\,\orcidlink{0009-0001-1146-5247}}
\affiliation{Institute for Particle Physics, ETH Z\"urich, Z\"urich 8093, Switzerland}

\author{Xin Chen\,\orcidlink{0000-0003-4027-3305}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{{Kohei Chinone}\,\orcidlink{0009-0006-5128-7672}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Dhruv Chouhan\,\orcidlink{0009-0007-2664-0742}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Andrea Coccaro\,\orcidlink{0000-0003-2368-4559}}
\affiliation{INFN Sezione di Genova, Via Dodecaneso, 33--16146, Genova, Italy}

\author{Stephane D\'{e}bieux} % No ORCID
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Ansh Desai\,\orcidlink{0000-0002-5447-8304}}
\affiliation{University of Oregon, Eugene, OR 97403, USA}

\author{Sergey Dmitrievsky\,\orcidlink{0000-0003-4247-8697}}
\affiliation{Affiliated with an international laboratory covered by a cooperation agreement with CERN.}

\author{Radu Dobre\,\orcidlink{0000-0002-9518-6068}}
\affiliation{Institute of Space Science---INFLPR Subsidiary, Bucharest, Romania}

\author{Monica D’Onofrio\,\orcidlink{0000-0003-2408-5099}}
\affiliation{University of Liverpool, Liverpool L69 3BX, United Kingdom}

\author{Sinead Eley\,\orcidlink{0009-0001-1320-2889}}
\affiliation{University of Liverpool, Liverpool L69 3BX, United Kingdom}

\author{Yannick Favre} % No ORCID
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Deion Fellers\,\orcidlink{0000-0002-0731-9562}}
\affiliation{University of Oregon, Eugene, OR 97403, USA}

\author{Jonathan~L.~Feng\,\orcidlink{0000-0002-7713-2138}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Carlo Alberto Fenoglio\,\orcidlink{0009-0007-7567-8763}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Didier Ferrere\,\orcidlink{0000-0002-5687-9240}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Max Fieg\,\orcidlink{0000-0002-7027-6921}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Wissal Filali\,\orcidlink{0009-0008-6961-2335}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Elena Firu\,\orcidlink{0000-0002-3109-5378}}
\affiliation{Institute of Space Science---INFLPR Subsidiary, Bucharest, Romania}

\author{{Haruhi Fujimori}\,\orcidlink{0009-0002-5026-8497}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Edward Galantay\,\orcidlink{0009-0001-6749-7360}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Ali Garabaglu\,\orcidlink{0000-0002-8105-6027}}
\affiliation{Department of Physics, University of Washington, PO Box 351560, Seattle, WA 98195-1460, USA}

\author{Stephen Gibson\,\orcidlink{0000-0002-1236-9249}}
\affiliation{Royal Holloway, University of London, Egham, TW20 0EX, United Kingdom}

\author{Sergio Gonzalez-Sevilla\,\orcidlink{0000-0003-4458-9403}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Yuri Gornushkin\,\orcidlink{0000-0003-3524-4032}}
\affiliation{Affiliated with an international laboratory covered by a cooperation agreement with CERN.}

\author{Carl Gwilliam\,\orcidlink{0000-0002-9401-5304}}
\affiliation{University of Liverpool, Liverpool L69 3BX, United Kingdom}

\author{Daiki Hayakawa\,\orcidlink{0000-0003-4253-4484}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Michael Holzbock\,\orcidlink{0000-0001-8018-4185}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Shih-Chieh Hsu\,\orcidlink{0000-0001-6214-8500}}
\affiliation{Department of Physics, University of Washington, PO Box 351560, Seattle, WA 98195-1460, USA}

\author{Zhen Hu\,\orcidlink{0000-0001-8209-4343}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{Giuseppe Iacobucci\,\orcidlink{0000-0001-9965-5442}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Tomohiro Inada\,\orcidlink{0000-0002-6923-9314}}
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Luca Iodice\,\orcidlink{0000-0002-3516-7121}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Sune Jakobsen\,\orcidlink{0000-0002-6564-040X}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Hans Joos\,\orcidlink{0000-0003-4313-4255}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}
\affiliation{II.~Physikalisches Institut, Universität Göttingen, Göttingen, Germany}

\author{Enrique Kajomovitz\,\orcidlink{0000-0002-8464-1790}}
\affiliation{Department of Physics and Astronomy, Technion---Israel Institute of Technology, Haifa 32000, Israel}

\author{{Takumi Kanai}\,\orcidlink{0009-0005-6840-4874}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Hiroaki Kawahara\,\orcidlink{0009-0007-5657-9954}}
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Alex Keyken\,\orcidlink{0009-0001-4886-2924}}
\affiliation{Royal Holloway, University of London, Egham, TW20 0EX, United Kingdom}

\author{Felix Kling\,\orcidlink{0000-0002-3100-6144}}
\affiliation{Deutsches Elektronen-Synchrotron DESY, Notkestr.~85, 22607 Hamburg, Germany}

\author{Daniela Köck\,\orcidlink{0000-0002-9090-5502}}
\affiliation{University of Oregon, Eugene, OR 97403, USA}

\author{Pantelis Kontaxakis\,\orcidlink{0000-0002-4860-5979}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Umut Kose\,\orcidlink{0000-0001-5380-9354}}
\affiliation{Institute for Particle Physics, ETH Z\"urich, Z\"urich 8093, Switzerland}

\author{Rafaella Kotitsa\,\orcidlink{0000-0002-7886-2685}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Peter Krack\,\orcidlink{0009-0003-5694-887X}}
\affiliation{Nikhef National Institute for Subatomic Physics, Science Park 105, 1098 XG Amsterdam, Netherlands}

\author{Susanne Kuehn\,\orcidlink{0000-0001-5270-0920}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Thanushan Kugathasan\,\orcidlink{0000-0003-4631-5019}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Lorne Levinson\,\orcidlink{0000-0003-4679-0485}}
\affiliation{Department of Particle Physics and Astrophysics, Weizmann Institute of Science, Rehovot 76100, Israel}

\author{Botao Li\,\orcidlink{0009-0009-0097-3367}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

\author{Jinfeng Liu\,\orcidlink{0000-0001-6827-1729}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{Yi Liu\,\orcidlink{0000-0002-3576-7004}}
\affiliation{School of Physics, Zhengzhou University, Zhengzhou 450001, China}

\author{Margaret~S.~Lutz\,\orcidlink{0000-0003-4515-0224}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Jack MacDonald\,\orcidlink{0000-0002-3150-3124}}
\affiliation{Institut f\"ur Physik, Universität Mainz, Mainz, Germany}

\author{Chiara Magliocca\,\orcidlink{0009-0009-4927-9253}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Toni~M\"akel\"a\,\orcidlink{0000-0002-1723-4028}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Lawson McCoy\,\orcidlink{0009-0009-2741-3220}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Josh McFayden\,\orcidlink{0000-0001-9273-2564}}
\affiliation{Department of Physics \& Astronomy, University of Sussex, Sussex House, Falmer, Brighton, BN1 9RH, United Kingdom}

\author{Andrea Pizarro Medina\,\orcidlink{0000-0002-1024-5605}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Matteo Milanesio\,\orcidlink{0000-0001-8778-9638}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Théo Moretti\,\orcidlink{0000-0001-7065-1923}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{{Keiko Moriyama\,\orcidlink{0009-0005-6447-2060}}} 
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Mitsuhiro Nakamura\,\orcidlink{0009-0002-6032-2741}}
\affiliation{Nagoya University, Furo-cho, Chikusa-ku, Nagoya 464-8602, Japan}

\author{Toshiyuki Nakano\,\orcidlink{0009-0004-8568-9077}}
\affiliation{Nagoya University, Furo-cho, Chikusa-ku, Nagoya 464-8602, Japan}

\author{Laurie Nevay\,\orcidlink{0000-0001-7225-9327}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{{Motoya Nonaka}\,\orcidlink{0009-0002-9433-2462}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{{Yuma Ohara}\,\orcidlink{0009-0005-7234-6718}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Ken Ohashi\,\orcidlink{0009-0000-9494-8457}}
\affiliation{Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics, University of Bern, Sidlerstrasse 5, CH-3012 Bern, Switzerland}

\author{{Kazuaki Okui}\,\orcidlink{0009-0002-3001-5310}}
\affiliation{Department of Physics, Chiba University, 1-33 Yayoi-cho Inage-ku, 263-8522 Chiba, Japan}

\author{Hidetoshi Otono\,\orcidlink{0000-0003-0760-5988}}
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Hao Pang\,\orcidlink{0000-0002-1946-1769}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{Lorenzo Paolozzi\,\orcidlink{0000-0002-9281-1972}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Pawan Pawan\,\orcidlink{0009-0004-9339-5984}}
\affiliation{University of Liverpool, Liverpool L69 3BX, United Kingdom}

\author{Brian Petersen\,\orcidlink{0000-0002-7380-6123}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Titi Preda,\orcidlink{0000-0002-5861-9370}}
\affiliation{Institute of Space Science---INFLPR Subsidiary, Bucharest, Romania}

\author{Markus Prim\,\orcidlink{0000-0002-1407-7450}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Michaela Queitsch-Maitland\,\orcidlink{0000-0003-4643-515X}}
\affiliation{University of Manchester, School of Physics and Astronomy, Schuster Building, Oxford Rd, Manchester M13 9PL, United Kingdom}

\author{Juan Rojo\,\orcidlink{0000-0003-4279-2192}}
\affiliation{Nikhef National Institute for Subatomic Physics, Science Park 105, 1098 XG Amsterdam, Netherlands}

\author{Hiroki Rokujo\,\orcidlink{0000-0002-3502-493X}}
\affiliation{Kyushu University, 744 Motooka, Nishi-ku, 819-0395 Fukuoka, Japan}

\author{Andr\'e Rubbia\,\orcidlink{0000-0002-5747-1001}}
\affiliation{Institute for Particle Physics, ETH Z\"urich, Z\"urich 8093, Switzerland}

\author{Jorge Sabater-Iglesias\,\orcidlink{0000-0003-2328-1952}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Osamu Sato\,\orcidlink{0000-0002-6307-7019}}
\affiliation{Nagoya University, Furo-cho, Chikusa-ku, Nagoya 464-8602, Japan}

\author{Paola Scampoli\,\orcidlink{0000-0001-7500-2535}}
\affiliation{Albert Einstein Center for Fundamental Physics, Laboratory for High Energy Physics, University of Bern, Sidlerstrasse 5, CH-3012 Bern, Switzerland}
\affiliation{Dipartimento di Fisica ``Ettore Pancini'', Universit\`a di Napoli Federico II, Complesso Universitario di Monte S.~Angelo, I-80126 Napoli, Italy}

\author{Kristof Schmieden\,\orcidlink{0000-0003-1978-4928}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Matthias Schott\,\orcidlink{0000-0002-4235-7265}}
\affiliation{Universit\"at Bonn, Regina-Pacis-Weg 3, D-53113 Bonn, Germany}

\author{Christiano Sebastiani\,\orcidlink{0000-0003-1073-035X}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Anna Sfyrla\,\orcidlink{0000-0002-3003-9905}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Davide Sgalaberna\,\orcidlink{0000-0001-6205-5013}}
\affiliation{Institute for Particle Physics, ETH Z\"urich, Z\"urich 8093, Switzerland}

\author{Mansoora Shamim\,\orcidlink{0009-0002-3986-399X}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Savannah Shively\,\orcidlink{0000-0002-4691-3767}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Yosuke Takubo\,\orcidlink{0000-0002-3143-8510}}
\affiliation{National Institute of Technology (KOSEN), Niihama College, 7-1, Yakumo-cho Niihama, 792-0805 Ehime, Japan}

\author{Noshin Tarannum\,\orcidlink{0000-0002-3246-2686}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Ondrej Theiner\,\orcidlink{0000-0002-6558-7311}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Simon Thor\,\orcidlink{0000-0002-9183-526X}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

\author{Eric Torrence\,\orcidlink{0000-0003-2911-8910}}
\affiliation{University of Oregon, Eugene, OR 97403, USA}

\author{Oscar Ivan Valdes Martinez\,\orcidlink{0000-0002-7314-7922}}
\affiliation{University of Manchester, School of Physics and Astronomy, Schuster Building, Oxford Rd, Manchester M13 9PL, United Kingdom}

\author{Svetlana Vasina\,\orcidlink{0000-0003-2775-5721}}
\affiliation{Affiliated with an international laboratory covered by a cooperation agreement with CERN.}

\author{Benedikt Vormwald\,\orcidlink{0000-0003-2607-7287}}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Yuxiao Wang\,\orcidlink{0009-0004-1228-9849}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{Eli Welch\,\orcidlink{0000-0001-6336-2912}}
\affiliation{Department of Physics and Astronomy, University of California, Irvine, CA 92697-4575, USA}

\author{Monika Wielers\,\orcidlink{0000-0001-9232-4827}}
\affiliation{Particle Physics Department, STFC Rutherford Appleton Laboratory, Harwell Campus, 
Didcot, OX11 0QX, United Kingdom}

\author{Benjamin James Wilson\,\orcidlink{0000-0002-7811-7474}}
\affiliation{University of Manchester, School of Physics and Astronomy, Schuster Building, Oxford Rd, Manchester M13 9PL, United Kingdom}

\author{Jialin Wu\,\orcidlink{0009-0001-6447-0410}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

\author{Johannes Martin Wuthrich\,\orcidlink{0000-0002-7522-8160}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

\author{Yue Xu\,\orcidlink{0000-0001-9563-4804}}
\affiliation{Department of Physics, University of Washington, PO Box 351560, Seattle, WA 98195-1460, USA}

%\author{Samuel Zahorec\,\orcidlink{0009-0000-9729-0611}}
%\affiliation{CERN, CH-1211 Geneva 23, Switzerland}
%\affiliation{Charles University, Faculty of Mathematics and Physics, Prague, Czech Republic}

\author{Stefano Zambito\,\orcidlink{0000-0002-4499-2545}}
\affiliation{D\'epartement de Physique Nucl\'eaire et Corpusculaire, University of Geneva, CH-1211 Geneva 4, Switzerland}

\author{Shunliang Zhang\,\orcidlink{0009-0001-1971-8878}}
\affiliation{Department of Physics, Tsinghua University, Beijing, China}

\author{Xingyu Zhao\,\orcidlink{0000-0003-1348-5732} \PRE{\vspace*{0.1in}}}
\affiliation{ETH Zurich, 8092 Zurich, Switzerland}

